LIMA: Less Is More for Alignment

Large language models are trained in two stages: (1) unsupervised pretraining from raw text, to learn general-purpose representations, and (2) large scale instruction tuning and reinforcement learning, to better align to end tasks and user preferences. We measure the relative importance of these two stages by training LIMA, a 65B parameter LLaMa language model fine-tuned with the standard supervised loss on only 1,000 carefully curated prompts and responses, without any reinforcement learning or human preference modeling. LIMA demonstrates remarkably strong performance, learning to follow specific response formats from only a handful of examples in the training data, including complex queries that range from planning trip itineraries to speculating about alternate history. Moreover, the model tends to generalize well to unseen tasks that did not appear in the training data. In a controlled human study, responses from LIMA are either equivalent or strictly preferred to GPT-4 in 43% of cases; this statistic is as high as 58% when compared to Bard and 65% versus DaVinci003, which was trained with human feedback. Taken together, these results strongly suggest that almost all knowledge in large language models is learned during pretraining, and only limited instruction tuning data is necessary to teach models to produce high quality output.

==> 07_related.tex <==
\section{Related Work}

Alignment techniques, particularly supervised fine-tuning~\citep{askell2021general,ouyang2022training}, have witnessed remarkable advancements in their ability to effectively leverage the knowledge within large models and enhance human interaction in natural language. The latest studies have predominantly concentrated on investigating alignment techniques in the creation of supervised instruction data~\citep{honovich2022unnatural} and different choices of large language models (e.g.,~\citep{touvron2023llama}). %\omer{I don't understand the second half of this sentence}\pfliu{rewording a little bit but feel free to make further edit}
The commonality of these works lies in either using OpenAI products (e.g., ChatGPT)\footnote{\url{https://chat.openai.com/}} to \emph{distill} instructions~\citep{alpaca,vicuna2023} or using a large number of instructions for supervised fine-tuning~\citep{beeching2023stackllama,sun2023principledriven,openassistant}.
For example, Alpaca~\citep{alpaca} underwent fine-tuning using 52,000 self-instructed instructions~\citep{wang2022selfinstruct}. 
% In the case of Dolly~\cite{XX}, it was trained on approximately 15,000 pairs of instruction and response records provided by Databricks employees across various domains. 
StackLLaMA~\citep{beeching2023stackllama}, on the other hand, relied on 10 million instructions from StackExchange and employed LLaMa 7B for training. OpenAssistant~\citep{openassistant} was trained using roughly 160,000 messages containing assistant-style conversations, which were both generated and annotated by humans.
% Vicuna-13B~\cite{XX}, an open-source chatbot, utilized fine-tuning with LLaMA on 70,000 conversations contributed by ChatGPT users. 


% \omer{We should call out distillation directly}\pfliu{fixed}

% \omer{We're not comparing with all that stuff...} \pfliu{compress a little}

In this paper, we are particularly concerned about the impact of data quality on fine-tuning, as well as how to manually construct high-quality data without relying on existing commercial products (e.g., ChatGPT) as assistance. This enables researchers to gain a more accurate understanding of alignment techniques through fine-tuning and efficiently find solutions in alignment applications in new scenarios.

\omer{missing: constitutional} 
% add unnatural self-*}



==> BACKUP_06_fewshot.tex <==
\section{Pretrained Models Quickly Learn New Tasks}

After demonstrating that LIMA is competent in a variety of question-answering and text generation tasks, we now test the boundaries of what can be achieved with only 1,000 examples.
We challenge LIMA in both multi-turn dialogue and text generation with structural constraints, and discover that LIMA exhibits surprising levels of robustness to these new tasks, and that even a handful of related training examples can dramatically boost its capabilities.


\subsection{Multi-Turn Dialogue}

Can a model fine-tuned on only 1,000 single-turn interactions engage in multi-turn dialogue?
We test LIMA across 10 live conversations, labeling each response as \textit{Fail}, \textit{Pass}, or \textit{Excellent} (see Section~\ref{sec:analysis}).
LIMA responses are surprisingly coherent for a zero-shot chatbot, referencing information from previous steps in the dialogue.
It is clear though that the model is operating out of distribution; in 6 out of 10 conversations, LIMA fails to follow the prompt within 3 interactions.

To improve its ability to converse, we gather 30 multi-turn dialogue chains.
Among these, 10 dialogues are composed by the authors, while the remaining 20 are based on comment chains from Stack Exchange, which we manually edit to fit the style of an assistant.
We fine-tune a new version of LIMA from the pretrained LLaMa model using the combined 1,030 examples, and conduct 10 live conversations based on the same prompts used for the zero-shot model.
Figure~\ref{fig:dialogue} shows excerpts from such dialogues.

Figure~\ref{fig:dialogue_results} shows the distribution of response quality before and after adding 30 examples of dialogue.
We observe that adding conversations substantially improves generation quality, raising the proportion of excellent responses from 45.2\% to 76.1\%.
Moreover, the failure rate drops from 15 fails per 42 turns (zero-shot) to 1 fail per 46 (fine-tuned).
We further compare the quality of the entire dialogue, and find that the fine-tuned model was significantly better in 7 out of 10 conversations, and tied with the zero-shot model in 3.
This leap in capability from a mere 30 examples, as well as the fact that the zero-shot model can converse at all, reinforces the hypothesis that such capabilities are learned during pretraining, and can be invoked through limited supervision.

\begin{wrapfigure}{r}{0.25\textwidth}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/multiturn_bar.pdf}
  \end{center}
  \caption{Analysis of dialogue turns, averaged over 10 test chats.}
  \label{fig:dialogue_results}
\end{wrapfigure}

\input{tables/dialogue}


\subsection{Generating Text with Complex Structure}

\omer{review}

In our preliminary experiments, we find that although LIMA can respond to many questions in our development set well, it cannot consistently respond to questions that specify the structures of the answer well, e.g. summarizing an article into bullet points or writing an article consisting of several key elements. 
Hence we investigate whether adding a few training examples of such question-answer pairs can help LIMA generalize to these tasks. 
We added six examples with format constraints, such as generating a product page that includes [highlights], [about the product], and [how to use] and generating QA pairs based on an article.

After training with these additional six examples, we test the model on a few questions with format constraints and surprisingly find that the responses of LIMA on such question are greatly improved. We present two generation examples in Table~\ref{fig:structure_examples}, from which we can see that LIMA failed to generate proper answers without any training examples that have format constraints in the question (left column), but it can generate remarkable examples of marketing plan given that we don't have any examples of marketing plans in the training data; in addition, it can summarize text into bullet points following user intents (right column).

% \begin{itemize}
%     \item Two examples that output a table based on the information from an article
%     \item one example of generating a paper review that includes sections of summary, strengths, weaknesses, potential.
%     \item One example of generating a product page that includes [highlights], [about the product], and [how to use].
% \end{itemize}


\input{tables/structure_output}




==> tables/ablation.tex <==
% \begin{figure}[t]
% \minipage{0.33\textwidth}
%   \includegraphics[width=\linewidth]{figs/quality.pdf}
%   \caption{(a) Quality}\label{fig:quality}
% \endminipage\hfill
% \minipage{0.33\textwidth}
%   \includegraphics[width=\linewidth]{figs/quantity.pdf}
%   \caption{(b) Quantity}\label{fig:quantity}
% \endminipage\hfill
% \minipage{0.33\textwidth}%
%   \includegraphics[width=\linewidth]{figs/diversity.pdf}
%  \caption{(c) Diversity}\label{fig:diversity}
% \endminipage
%   \caption{Ablations on the effects of supervised fine-tuning data w.r.t. quality, quantity and diversity.
% \label{fig:abl}}
% \end{figure}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.323\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figs/ppl_7b.pdf}
         \caption{LIMA 7B}
         \label{fig:ppl:7b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.323\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figs/ppl_30b.pdf}
         \caption{LIMA 30B}
         \label{fig:ppl:30b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.323\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figs/ppl_65b.pdf}
         \caption{LIMA 65B}
         \label{fig:ppl:65B}
     \end{subfigure}
        \caption{Validation PPL and generation quality evaluated by ChatGPT.}
        \label{fig:ppl}
\end{figure}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figs/quality_bar.pdf}
         \caption{Different training data. \omer{add error bars / confidence interval / boxplot}}
         \label{fig:quality}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figs/quantity_se.pdf}
         \caption{Varying training data size on SE. \omer{here too}}
         \label{fig:ppl:65B}
     \end{subfigure}
        \caption{Ablation studies.}
        \label{fig:abl}
\end{figure}

% \pfliu{
%         (1) Figure (a): Does generation quality refer to the likert score (1-6) in automatic evaluation in y-axis, and what do D1, D2, D3 and D4 in represent?  (2) Figure (b) : How are quality and diversity controlled as quantity increases
%         (3) Figure (c) : Similarly, is the x-axis means that the effect 
%  of one specific domain (e.g., Full SE)? Similarly, how are the,quality and quantity quantities controlled in this situation
%  (4) add which model (7B or 30B) is used. (5) we potentially could break down the overall generation quality in terms of different scenarios (e.g., writing, math, code etc)}
